Dependency-aware Resource Allocation for Serverless Functions at the Edge

Serverless computing allows developers to break their code into small components, known as functions, which are automatically managed by a service provider. Being lightweight and modular, serverless functions have been increasingly employed in edge computing, where quick responses and adaptability are key to meeting strict latency requirements. In particular, edge nodes are intrinsically resource-constrained, and efficient resource allocation strategies are crucial for optimizing their usage. Different approaches exist in the literature, but they often overlook the dependencies among functions, that is, how and when functions invoke other functions, obtaining suboptimal results. This paper presents NEPTUNE+, a dependency-aware resource (CPU cores) allocation solution for serverless functions deployed at the edge. The approach extends NEPTUNE, an existing framework for managing edge infrastructures, with a new theoretical model and control algorithm that take dependencies into account function. We evaluated NEPTUNE+ by using three applications and it is able to allocate up to 42% fewer cores compared to NEPTUNE.

==> sections/discussion.tex <==
From the results of our experiments, we observed that the percentage of core allocation difference between solutions that do not support dependencies like NP and our solution NP$^+$ does not have a linear factor. Many factories influence this difference such as the complexity of the application, number of functions suffering from bottleneck, and the magnitude of the bottlenecks. The higher are these factories, the higher will be the percentage difference, however, a balance might be done between the factories. 
Back to our statistical results, Our solution allocated 23\% millicores less than NP in \textit{hotel reservation} application, 24\% for \textit{shock-shop} and 35\% for the \textit{complex} application. We have this differences because of the complexity of the applications. \textit{Hotel reservation} is less complex than \textit{shock-shop}, and \textit{shock-shop} is less than the \textit{complex} application.
When we simulated bottlenecks, NP$^+$ allocated 40\% millicores less than NP in \textit{hotel reservation} application, 30\% for \textit{shock-shop} and 42\% for the \textit{complex} application. With bottleneck, the core allocation percentage difference was higher in \textit{hotel reservation} than in \textit{shock-shop} because although \textit{shock-shop} is more complex than \textit{hotel reservation} the magnitude of workload simulated for the bottleneck in \textit{hotel reservation} was very higher, range of 800-6000 requests, while for \textit{shock-shop} we simulated from 400-2400 requests.

==> sections/references.tex <==
\bibliographystyle{plain}
\bibliography{sections/ref}

==> sections/serverlessFunctionsEdge.tex <==
Serverless computing is an innovative and promising technology that is revolutionizing application development, deployment and execution by eliminating the need for developers to manage infrastructure thereby enhancing developer productivity; service providers reducing costs in infrastructure and servers management while, end-users reduce costs for running applications on pay-as-you-go base thanks to autoscaling.
\par
Serverless computing makes cloud computing (seen by users as infinity resource pool) even more powerful and suitable to run complex applications, however, due to the network latency, cloud computing might not be a good choice for very low latency demanding applications therefore emerged edge computing. 
\par
Edge computing is a new computing architecture which the infrastructure is placed at the edge of the network where the user produce data. Edge computing is typically designed to meet the extremely low latency applications requirements that is almost impossible to be met on the cloud. 
\par
While cloud has "infinity" resources, edge is known as resource constrained implying many challenges. The main question when adopting edge computing is \textit{how do we guarantee an efficient resource management?} To tackle this problem, many approaches including autoscaling \cite{raith2022mobilityServFunct}, service placement optimization \cite{yussupov2019systematicReviewTools} have been proposed by researchers but are not comprehensive solutions. In NEPTUNE \cite{baresi2022neptune} was addressed a comprehensive edge computing architecture which explore serverless computing paradigm for complex applications taking into account serverless functions placement, user requests routing and network delays. Was considered parallelization of complex applications by launching serverless functions instances to the GPU if available. While other approaches are partial solutions by considering single or few aspects, NEPTUNE is a holistic solution tackling all the aspects from deployment to run-time management.
\par
In NEPTUNE architecture, distributed nodes are made accessible the users to deploy and execute there applications. According to the end-users mobility and workload, some requests are forwarded to the nearest nodes.
\subsection{Deployment}
An application is deployed as a set of serverless functions; for each function, the following elements are required for deployment process: function's code, response time threshold (known as service level agreement-SLA) and RAM needed to properly execute the function.
After deployment, NEPTUNE performs the whole following function execution process including generation and replication of functions instances, routing, core allocation to fulfill the expected response time.  
\subsection{Serverless Functions Management}
The functions are managed in three hierarchical levels: topology, community and node. 
\par
\textbf{Topology Level}. This is the highest level in the hierarchy which is in charge of creating and managing communities of nodes and making them isolated and independent from each other. The isolation of the communities is to avoid the node resources contention that can be caused by communities overlapping. 
\par
\textbf{Community Level}. Manages nodes resources and computes routing protocols and policies, enabling nodes to forward some requests to the closest node within the community. From the communities polices, the nodes are also aware about computation-intensive functions and they forward requests to GPU if available. 
\par
\textbf{Node Level}. This is the lowest level of NEPTUNE architecture and is the one that guarantee the execution of the functions. Node level ensures that each function instance has enough resources including number of cores to finish its execution within the given SLA.
\subsection{Core Allocation in NEPTUNE}
\label{sec:nepCoreAlloc}
The core allocation process is managed on the node level taking into account the management of the turnaround time of requested task.\footnote{Overall time to complete a requested task, counting from requesting instant until the last response delivery.}
Because the network delay is managed by the community level, the node level is in charge of adjusting the queue and execution times QE. QE is mainly influenced by the number of requests for a specific function and the execution environment. To adjust the QE and therefore, fulfill the SLA we change the amount of cores allocated to the function instance. The core allocation is dynamic and automatically done using control theoretical approach, a lightweight Proportional Integer (PI) controller. The cores for each function instance are managed by an independent and isolated PI controller. 
Given a function instance \textit{f} and its desired response time SLA\textsubscript{f}, in a specific node, we define a set point value QE\textsubscript{f\textsubscript{control}} (QE\textsubscript{f\textsubscript{control}}\textless \ SLA\textsubscript{f})for the PI controller. In fig.~\ref{fig:controller_neptune} we present function instance response time management scenario in runtime.  
\par
\begin{figure}[H]
  \centering
  \includegraphics[width=0.55\textwidth]{sections/images/control_neptune_graph.pdf}
  \caption{Theoretical approach, function instance response time management in runtime}
  \label{fig:controller_neptune}
\end{figure}
The PI controller is monitoring a function instance queue and execution times QE\textsubscript{f} and adjusting to keep in the set point of the controller  QE\textsubscript{f\textsubscript{control}}. In the graph of fig.~\ref{fig:controller_neptune} the controller take action in four control times ct where the delta between QE\textsubscript{f} and QE\textsubscript{f\textsubscript{control}} was increasing than expected. As previously discussed, to adjust the QE\textsubscript{f} the controller increase or reduce the amount of cores. The number of cores is increased when the QE\textsubscript{f} goes above the QE\textsubscript{f\textsubscript{control}} and decrease when goes below. This control procedure is performed in the whole life of each function instance, avoiding violations of desired function response time SLA\textsubscript{f}.

\subsection{Problem Statement}
\label{sec:problemstatement}

Given F, a set of dependent serverless functions represented by DAG D\textsubscript{\textit{f}} = (N\textsubscript{\textit{f}}, E\textsubscript{\textit{f}}) as described in section \ref{sec:functionDepModel}. In the state-of-the-art the controller monitors the response time of each function $\textit{f}\textsubscript{i} \in F$ considering  that all \textit{f}\textsubscript{i} work isolated from each other leading to inefficiency cores allocation.
Let F be a set of functions \textit{f}\textsubscript{1}, \textit{f}\textsubscript{2} and \textit{f}\textsubscript{3} with dependencies $\textit{f}\textsubscript{1} \rightarrow \textit{f}\textsubscript{2}\rightarrow \textit{f}\textsubscript{3})$, \textit{f}\textsubscript{3} is a child of \textit{f}\textsubscript{2} and \textit{f}\textsubscript{2} a child of \textit{f}\textsubscript{1} ( \textit{f}\textsubscript{1} depends on \textit{f}\textsubscript{2} and \textit{f}\textsubscript{2} on \textit{f}\textsubscript{3}). Beside dependencies, also consider that each function as its own code (local code) to be executed. Now, Let each function \textit{f}\textsubscript{i} be defined as (\textit{lcode}\textsubscript{\textit{f}\textsubscript{i}}, \textit{children}\textsubscript{\textit{f}\textsubscript{i}}) where \textit{lcode}\textsubscript{\textit{f}\textsubscript{i}} is the local code of \textit{f}\textsubscript{i} and \textit{children}\textsubscript{\textit{f}\textsubscript{i}} the set of functions of  \textit{f}\textsubscript{i}. Given a number of requests \textit{r}\textsubscript{i} to \textit{f}\textsubscript{i}, \textit{lcode}\textsubscript{\textit{f}\textsubscript{i}} has its response time (local response time)\footnote{Time needed for local code execution.} and each child from \textit{children}\textsubscript{\textit{f}\textsubscript{i}} as well (external response time)\footnote{Time needed for called function execution.}. Let  \textit{lrt}\textsubscript{\textit{f}\textsubscript{i}} be the local response time of \textit{f}\textsubscript{i} and \textit{exrt}\textsubscript{\textit{f}\textsubscript{i}} the total external response time of \textit{f}\textsubscript{i}. 
\par
Let \textit{s}\textsubscript{\textit{f}\textsubscript{i}} be a set of functions that \textit{f}\textsubscript{i} calls in sequential way and with no parallelism with other functions in \textit{f}\textsubscript{i}. Let  \textit{s}\textsubscript{\textit{j}\textit{f}\textsubscript{i}} be each function of \textit{s}\textsubscript{\textit{f}\textsubscript{i}}, $\textit{s}\textsubscript{\textit{j}\textit{f}\textsubscript{i}} \in \textit{s}\textsubscript{\textit{f}\textsubscript{i}}$ and \textit{grt}\textsubscript{\textit{s}\textsubscript{\textit{j}\textit{f}\textsubscript{i}}} the global response time of \textit{s}\textsubscript{\textit{j}\textit{f}\textsubscript{i}}.
\par
Let \textit{p}\textsubscript{\textit{f}\textsubscript{i}} be a set of functions called in parallel with some other functions in  \textit{f}\textsubscript{i}. Let \textit{s}\textsubscript{\textit{sync}k\textit{f}\textsubscript{i}} be a set of parallel functions called in parallel, and k (which is the same for a particular set of functions) defines the sequence of call,  $\textit{s}\textsubscript{\textit{sync}k\textit{f}\textsubscript{i}} \in  \textit{p}\textsubscript{\textit{f}\textsubscript{i}}$ and \textit{grt}\textsubscript{\textit{s}\textsubscript{\textit{sync}k\textit{f}\textsubscript{i}}} the global response time of \textit{s}\textsubscript{\textit{sync}k\textit{f}\textsubscript{i}}
We get the external response time by the formula \ref{eq:exrt}:

\begin{equation}
\textit{exrt}\textsubscript{\textit{f}\textsubscript{i}}=\sum_{j=1}^{n}(\textit{grt}\textsubscript{\textit{s}\textsubscript{\textit{j}\textit{f}\textsubscript{i}}}) + \sum_{k=1}^{n} Max(\textit{grt}\textsubscript{\textit{s}\textsubscript{\textit{sync}k\textit{f}\textsubscript{i}}}) : \   i \ is\ a \ constant\ in\ N
\label{eq:exrt}
\end{equation}
Then the global response time of  \textit{f}\textsubscript{i}, \textit{grt}\textsubscript{\textit{f}\textsubscript{i}} is given by expression \ref{eq:trt} as a sum of local response time and total external response time: 
\begin{equation}
\textit{grt}\textsubscript{\textit{f}\textsubscript{i}}=\textit{lrt}\textsubscript{\textit{f}\textsubscript{i}}+\textit{exrt}\textsubscript{\textit{f}\textsubscript{i}}
\label{eq:trt}
\end{equation}
To keep acceptable global response time of each serverless function \textit{f}\textsubscript{i}, user provides SLA for it and the service provider must keep the \textit{grt}\textsubscript{\textit{f}\textsubscript{i}} in a way that cannot violet the given SLA. This is done by adopting the control theory approach(e.g.: see section \ref{sec:nepCoreAlloc}). In the state-of-the-art including \cite{baresi2022neptune} the controller placed in each node, monitors the global response time increasing the number of cores when the \textit{grt}\textsubscript{\textit{f}\textsubscript{i}} goes above the set point value or decreasing number of cores when the \textit{grt}\textsubscript{\textit{f}\textsubscript{i}} goes bellow the set point.
Considering the set of functions $\textit{f}\textsubscript{1} \rightarrow \textit{f}\textsubscript{2}\rightarrow \textit{f}\textsubscript{3})$, where each function as its global response time, \textit{grt}\textsubscript{\textit{f}\textsubscript{1}}, \textit{grt}\textsubscript{\textit{f}\textsubscript{2}} and \textit{grt}\textsubscript{\textit{f}\textsubscript{3}}. Imagine a bottleneck on \textit{f}\textsubscript{3}, that means the \textit{grt}\textsubscript{\textit{f}\textsubscript{3}} will increase affecting the \textit{grt}\textsubscript{\textit{f}\textsubscript{2}} and in chain the \textit{grt}\textsubscript{\textit{f}\textsubscript{1}}. In the same way, the controllers of each function will react to keep the global response time aligned to the SLA of each function. The controller in \textsubscript{\textit{f}\textsubscript{3}} increases the number of cores as well in \textsubscript{\textit{f}\textsubscript{2}} and \textsubscript{\textit{f}\textsubscript{1}}. Note that in a very simple application, because of bottleneck in one function, we allocated cores three times more than necessary. In complex applications this problem can lead to a very high bill to be paid by the end-user, as well as high investment in equipment from the service providers. In edge computing, due to the resource constrain this issue can be even serious, therefore can make the application not working or, in extreme cases, the whole edge computing system.\par
To tackle this problem, we present NEPTUNE+, efficient resource allocation in dependent serverless functions.

